Neural Networks for Information Retrieval

Machine learning plays a role in many aspects of modern IR systems, and deep learning is applied in all of them. The fast pace of modern-day research has given rise to many different approaches for many different IR problems. The amount of information available can be overwhelming both for junior students and for experienced researchers looking for new research topics and directions. Additionally, it is interesting to see what key insights into IR problems the new technologies are able to give us. The aim of this full-day tutorial is to give a clear overview of current tried-and-trusted neural methods in IR and how they benefit IR research. It covers key architectures, as well as the most promising future directions.

==> LinLibertine_I.tex <==
\DeclareTextGlyphY{LinLibertine_I}{space}{32}
\DeclareTextGlyphY{LinLibertine_I}{uni0020}{32}
\DeclareTextGlyphY{LinLibertine_I}{zero}{48}
\DeclareTextGlyphY{LinLibertine_I}{uni0030}{48}
\DeclareTextGlyphY{LinLibertine_I}{one}{49}
\DeclareTextGlyphY{LinLibertine_I}{uni0031}{49}
\DeclareTextGlyphY{LinLibertine_I}{two}{50}
\DeclareTextGlyphY{LinLibertine_I}{uni0032}{50}
\DeclareTextGlyphY{LinLibertine_I}{three}{51}
\DeclareTextGlyphY{LinLibertine_I}{uni0033}{51}
\DeclareTextGlyphY{LinLibertine_I}{four}{52}
\DeclareTextGlyphY{LinLibertine_I}{uni0034}{52}
\DeclareTextGlyphY{LinLibertine_I}{five}{53}
\DeclareTextGlyphY{LinLibertine_I}{uni0035}{53}
\DeclareTextGlyphY{LinLibertine_I}{six}{54}
\DeclareTextGlyphY{LinLibertine_I}{uni0036}{54}
\DeclareTextGlyphY{LinLibertine_I}{seven}{55}
\DeclareTextGlyphY{LinLibertine_I}{uni0037}{55}
\DeclareTextGlyphY{LinLibertine_I}{eight}{56}
\DeclareTextGlyphY{LinLibertine_I}{uni0038}{56}
\DeclareTextGlyphY{LinLibertine_I}{nine}{57}
\DeclareTextGlyphY{LinLibertine_I}{uni0039}{57}
\DeclareTextGlyphY{LinLibertine_I}{A}{65}
\DeclareTextGlyphY{LinLibertine_I}{uni0041}{65}
\DeclareTextGlyphY{LinLibertine_I}{B}{66}
\DeclareTextGlyphY{LinLibertine_I}{uni0042}{66}
\DeclareTextGlyphY{LinLibertine_I}{C}{67}
\DeclareTextGlyphY{LinLibertine_I}{uni0043}{67}
\DeclareTextGlyphY{LinLibertine_I}{D}{68}
\DeclareTextGlyphY{LinLibertine_I}{uni0044}{68}
\DeclareTextGlyphY{LinLibertine_I}{E}{69}
\DeclareTextGlyphY{LinLibertine_I}{uni0045}{69}
\DeclareTextGlyphY{LinLibertine_I}{F}{70}
\DeclareTextGlyphY{LinLibertine_I}{uni0046}{70}
\DeclareTextGlyphY{LinLibertine_I}{G}{71}
\DeclareTextGlyphY{LinLibertine_I}{uni0047}{71}
\DeclareTextGlyphY{LinLibertine_I}{H}{72}
\DeclareTextGlyphY{LinLibertine_I}{uni0048}{72}
\DeclareTextGlyphY{LinLibertine_I}{I}{73}
\DeclareTextGlyphY{LinLibertine_I}{uni0049}{73}
\DeclareTextGlyphY{LinLibertine_I}{J}{74}
\DeclareTextGlyphY{LinLibertine_I}{uni004A}{74}
\DeclareTextGlyphY{LinLibertine_I}{K}{75}
\DeclareTextGlyphY{LinLibertine_I}{uni004B}{75}
\DeclareTextGlyphY{LinLibertine_I}{L}{76}
\DeclareTextGlyphY{LinLibertine_I}{uni004C}{76}
\DeclareTextGlyphY{LinLibertine_I}{M}{77}
\DeclareTextGlyphY{LinLibertine_I}{uni004D}{77}
\DeclareTextGlyphY{LinLibertine_I}{N}{78}
\DeclareTextGlyphY{LinLibertine_I}{uni004E}{78}
\DeclareTextGlyphY{LinLibertine_I}{O}{79}
\DeclareTextGlyphY{LinLibertine_I}{uni004F}{79}
\DeclareTextGlyphY{LinLibertine_I}{P}{80}
\DeclareTextGlyphY{LinLibertine_I}{uni0050}{80}
\DeclareTextGlyphY{LinLibertine_I}{Q}{81}
\DeclareTextGlyphY{LinLibertine_I}{uni0051}{81}
\DeclareTextGlyphY{LinLibertine_I}{R}{82}
\DeclareTextGlyphY{LinLibertine_I}{uni0052}{82}
\DeclareTextGlyphY{LinLibertine_I}{S}{83}
\DeclareTextGlyphY{LinLibertine_I}{uni0053}{83}
\DeclareTextGlyphY{LinLibertine_I}{T}{84}
\DeclareTextGlyphY{LinLibertine_I}{uni0054}{84}
\DeclareTextGlyphY{LinLibertine_I}{U}{85}
\DeclareTextGlyphY{LinLibertine_I}{uni0055}{85}
\DeclareTextGlyphY{LinLibertine_I}{V}{86}
\DeclareTextGlyphY{LinLibertine_I}{uni0056}{86}
\DeclareTextGlyphY{LinLibertine_I}{W}{87}
\DeclareTextGlyphY{LinLibertine_I}{uni0057}{87}
\DeclareTextGlyphY{LinLibertine_I}{X}{88}
\DeclareTextGlyphY{LinLibertine_I}{uni0058}{88}
\DeclareTextGlyphY{LinLibertine_I}{Y}{89}
\DeclareTextGlyphY{LinLibertine_I}{uni0059}{89}
\DeclareTextGlyphY{LinLibertine_I}{Z}{90}
\DeclareTextGlyphY{LinLibertine_I}{uni005A}{90}
\DeclareTextGlyphY{LinLibertine_I}{asciicircum}{94}
\DeclareTextGlyphY{LinLibertine_I}{uni005E}{94}
\DeclareTextGlyphY{LinLibertine_I}{Adieresis}{196}
\DeclareTextGlyphY{LinLibertine_I}{uni00C4}{196}
\DeclareTextGlyphY{LinLibertine_I}{Aring}{197}
\DeclareTextGlyphY{LinLibertine_I}{uni00C5}{197}
\DeclareTextGlyphY{LinLibertine_I}{AE}{198}
\DeclareTextGlyphY{LinLibertine_I}{uni00C6}{198}
\DeclareTextGlyphY{LinLibertine_I}{Ccedilla}{199}
\DeclareTextGlyphY{LinLibertine_I}{uni00C7}{199}
\DeclareTextGlyphY{LinLibertine_I}{Odieresis}{214}
\DeclareTextGlyphY{LinLibertine_I}{uni00D6}{214}
\DeclareTextGlyphY{LinLibertine_I}{Oslash}{216}
\DeclareTextGlyphY{LinLibertine_I}{uni00D8}{216}
\DeclareTextGlyphY{LinLibertine_I}{Udieresis}{220}
\DeclareTextGlyphY{LinLibertine_I}{uni00DC}{220}
\DeclareTextGlyphY{LinLibertine_I}{Thorn}{222}
\DeclareTextGlyphY{LinLibertine_I}{uni00DE}{222}
\DeclareTextGlyphY{LinLibertine_I}{iogonek}{303}
\DeclareTextGlyphY{LinLibertine_I}{uni012F}{303}
\DeclareTextGlyphY{LinLibertine_I}{IJ}{306}
\DeclareTextGlyphY{LinLibertine_I}{uni0132}{306}
\DeclareTextGlyphY{LinLibertine_I}{Eng}{330}
\DeclareTextGlyphY{LinLibertine_I}{uni014A}{330}
\DeclareTextGlyphY{LinLibertine_I}{Ohungarumlaut}{336}
\DeclareTextGlyphY{LinLibertine_I}{uni0150}{336}
\DeclareTextGlyphY{LinLibertine_I}{OE}{338}
\DeclareTextGlyphY{LinLibertine_I}{uni0152}{338}
\DeclareTextGlyphY{LinLibertine_I}{Uhungarumlaut}{368}
\DeclareTextGlyphY{LinLibertine_I}{uni0170}{368}
\DeclareTextGlyphY{LinLibertine_I}{Alpha}{913}
\DeclareTextGlyphY{LinLibertine_I}{uni0391}{913}
\DeclareTextGlyphY{LinLibertine_I}{Beta}{914}
\DeclareTextGlyphY{LinLibertine_I}{uni0392}{914}
\DeclareTextGlyphY{LinLibertine_I}{Gamma}{915}
\DeclareTextGlyphY{LinLibertine_I}{uni0393}{915}
\DeclareTextGlyphY{LinLibertine_I}{Delta}{916}
\DeclareTextGlyphY{LinLibertine_I}{uni0394}{916}
\DeclareTextGlyphY{LinLibertine_I}{Epsilon}{917}
\DeclareTextGlyphY{LinLibertine_I}{uni0395}{917}
\DeclareTextGlyphY{LinLibertine_I}{Zeta}{918}
\DeclareTextGlyphY{LinLibertine_I}{uni0396}{918}
\DeclareTextGlyphY{LinLibertine_I}{Eta}{919}
\DeclareTextGlyphY{LinLibertine_I}{uni0397}{919}
\DeclareTextGlyphY{LinLibertine_I}{Theta}{920}
\DeclareTextGlyphY{LinLibertine_I}{uni0398}{920}
\DeclareTextGlyphY{LinLibertine_I}{Iota}{921}
\DeclareTextGlyphY{LinLibertine_I}{uni0399}{921}
\DeclareTextGlyphY{LinLibertine_I}{Kappa}{922}
\DeclareTextGlyphY{LinLibertine_I}{uni039A}{922}
\DeclareTextGlyphY{LinLibertine_I}{Lambda}{923}
\DeclareTextGlyphY{LinLibertine_I}{uni039B}{923}
\DeclareTextGlyphY{LinLibertine_I}{Mu}{924}
\DeclareTextGlyphY{LinLibertine_I}{uni039C}{924}
\DeclareTextGlyphY{LinLibertine_I}{Nu}{925}
\DeclareTextGlyphY{LinLibertine_I}{uni039D}{925}
\DeclareTextGlyphY{LinLibertine_I}{Xi}{926}
\DeclareTextGlyphY{LinLibertine_I}{uni039E}{926}
\DeclareTextGlyphY{LinLibertine_I}{Omicron}{927}
\DeclareTextGlyphY{LinLibertine_I}{uni039F}{927}
\DeclareTextGlyphY{LinLibertine_I}{Pi}{928}
\DeclareTextGlyphY{LinLibertine_I}{uni03A0}{928}
\DeclareTextGlyphY{LinLibertine_I}{Rho}{929}
\DeclareTextGlyphY{LinLibertine_I}{uni03A1}{929}
\DeclareTextGlyphY{LinLibertine_I}{Sigma}{931}
\DeclareTextGlyphY{LinLibertine_I}{uni03A3}{931}
\DeclareTextGlyphY{LinLibertine_I}{Tau}{932}
\DeclareTextGlyphY{LinLibertine_I}{uni03A4}{932}
\DeclareTextGlyphY{LinLibertine_I}{Upsilon}{933}
\DeclareTextGlyphY{LinLibertine_I}{uni03A5}{933}
\DeclareTextGlyphY{LinLibertine_I}{Phi}{934}
\DeclareTextGlyphY{LinLibertine_I}{uni03A6}{934}
\DeclareTextGlyphY{LinLibertine_I}{Chi}{935}
\DeclareTextGlyphY{LinLibertine_I}{uni03A7}{935}
\DeclareTextGlyphY{LinLibertine_I}{Psi}{936}
\DeclareTextGlyphY{LinLibertine_I}{uni03A8}{936}
\DeclareTextGlyphY{LinLibertine_I}{Omega}{937}
\DeclareTextGlyphY{LinLibertine_I}{uni03A9}{937}
\DeclareTextGlyphY{LinLibertine_I}{Iotadieresis}{938}
\DeclareTextGlyphY{LinLibertine_I}{uni03AA}{938}
\DeclareTextGlyphY{LinLibertine_I}{Upsilon1}{978}
\DeclareTextGlyphY{LinLibertine_I}{uni03D2}{978}
\DeclareTextGlyphY{LinLibertine_I}{afii10051}{1026}
\DeclareTextGlyphY{LinLibertine_I}{uni0402}{1026}
\DeclareTextGlyphY{LinLibertine_I}{afii10053}{1028}
\DeclareTextGlyphY{LinLibertine_I}{uni0404}{1028}
\DeclareTextGlyphY{LinLibertine_I}{afii10054}{1029}
\DeclareTextGlyphY{LinLibertine_I}{uni0405}{1029}
\DeclareTextGlyphY{LinLibertine_I}{afii10055}{1030}
\DeclareTextGlyphY{LinLibertine_I}{uni0406}{1030}
\DeclareTextGlyphY{LinLibertine_I}{afii10056}{1031}
\DeclareTextGlyphY{LinLibertine_I}{uni0407}{1031}
\DeclareTextGlyphY{LinLibertine_I}{afii10057}{1032}
\DeclareTextGlyphY{LinLibertine_I}{uni0408}{1032}
\DeclareTextGlyphY{LinLibertine_I}{afii10058}{1033}
\DeclareTextGlyphY{LinLibertine_I}{uni0409}{1033}
\DeclareTextGlyphY{LinLibertine_I}{afii10059}{1034}
\DeclareTextGlyphY{LinLibertine_I}{uni040A}{1034}
\DeclareTextGlyphY{LinLibertine_I}{afii10060}{1035}
\DeclareTextGlyphY{LinLibertine_I}{uni040B}{1035}
\DeclareTextGlyphY{LinLibertine_I}{afii10061}{1036}
\DeclareTextGlyphY{LinLibertine_I}{uni040C}{1036}
\DeclareTextGlyphY{LinLibertine_I}{uni040D}{1037}
\DeclareTextGlyphY{LinLibertine_I}{afii10062}{1038}
\DeclareTextGlyphY{LinLibertine_I}{uni040E}{1038}
\DeclareTextGlyphY{LinLibertine_I}{afii10145}{1039}
\DeclareTextGlyphY{LinLibertine_I}{uni040F}{1039}
\DeclareTextGlyphY{LinLibertine_I}{afii10017}{1040}
\DeclareTextGlyphY{LinLibertine_I}{uni0410}{1040}
\DeclareTextGlyphY{LinLibertine_I}{afii10018}{1041}
\DeclareTextGlyphY{LinLibertine_I}{uni0411}{1041}
\DeclareTextGlyphY{LinLibertine_I}{afii10019}{1042}
\DeclareTextGlyphY{LinLibertine_I}{uni0412}{1042}
\DeclareTextGlyphY{LinLibertine_I}{afii10020}{1043}
\DeclareTextGlyphY{LinLibertine_I}{uni0413}{1043}
\DeclareTextGlyphY{LinLibertine_I}{afii10021}{1044}
\DeclareTextGlyphY{LinLibertine_I}{uni0414}{1044}
\DeclareTextGlyphY{LinLibertine_I}{afii10022}{1045}
\DeclareTextGlyphY{LinLibertine_I}{uni0415}{1045}
\DeclareTextGlyphY{LinLibertine_I}{afii10024}{1046}
\DeclareTextGlyphY{LinLibertine_I}{uni0416}{1046}
\DeclareTextGlyphY{LinLibertine_I}{afii10025}{1047}
\DeclareTextGlyphY{LinLibertine_I}{uni0417}{1047}
\DeclareTextGlyphY{LinLibertine_I}{afii10026}{1048}
\DeclareTextGlyphY{LinLibertine_I}{uni0418}{1048}
\DeclareTextGlyphY{LinLibertine_I}{afii10027}{1049}
\DeclareTextGlyphY{LinLibertine_I}{uni0419}{1049}
\DeclareTextGlyphY{LinLibertine_I}{afii10028}{1050}
\DeclareTextGlyphY{LinLibertine_I}{uni041A}{1050}
\DeclareTextGlyphY{LinLibertine_I}{afii10029}{1051}
\DeclareTextGlyphY{LinLibertine_I}{uni041B}{1051}
\DeclareTextGlyphY{LinLibertine_I}{afii10030}{1052}
\DeclareTextGlyphY{LinLibertine_I}{uni041C}{1052}
\DeclareTextGlyphY{LinLibertine_I}{afii10031}{1053}
\DeclareTextGlyphY{LinLibertine_I}{uni041D}{1053}
\DeclareTextGlyphY{LinLibertine_I}{afii10032}{1054}
\DeclareTextGlyphY{LinLibertine_I}{uni041E}{1054}
\DeclareTextGlyphY{LinLibertine_I}{afii10033}{1055}
\DeclareTextGlyphY{LinLibertine_I}{uni041F}{1055}
\DeclareTextGlyphY{LinLibertine_I}{afii10034}{1056}
\DeclareTextGlyphY{LinLibertine_I}{uni0420}{1056}
\DeclareTextGlyphY{LinLibertine_I}{afii10035}{1057}
\DeclareTextGlyphY{LinLibertine_I}{uni0421}{1057}
\DeclareTextGlyphY{LinLibertine_I}{afii10036}{1058}
\DeclareTextGlyphY{LinLibertine_I}{uni0422}{1058}
\DeclareTextGlyphY{LinLibertine_I}{afii10037}{1059}
\DeclareTextGlyphY{LinLibertine_I}{uni0423}{1059}
\DeclareTextGlyphY{LinLibertine_I}{afii10038}{1060}
\DeclareTextGlyphY{LinLibertine_I}{uni0424}{1060}
\DeclareTextGlyphY{LinLibertine_I}{afii10039}{1061}
\DeclareTextGlyphY{LinLibertine_I}{uni0425}{1061}
\DeclareTextGlyphY{LinLibertine_I}{afii10040}{1062}
\DeclareTextGlyphY{LinLibertine_I}{uni0426}{1062}
\DeclareTextGlyphY{LinLibertine_I}{afii10041}{1063}
\DeclareTextGlyphY{LinLibertine_I}{uni0427}{1063}
\DeclareTextGlyphY{LinLibertine_I}{afii10042}{1064}
\DeclareTextGlyphY{LinLibertine_I}{uni0428}{1064}
\DeclareTextGlyphY{LinLibertine_I}{afii10043}{1065}
\DeclareTextGlyphY{LinLibertine_I}{uni0429}{1065}
\DeclareTextGlyphY{LinLibertine_I}{afii10044}{1066}
\DeclareTextGlyphY{LinLibertine_I}{uni042A}{1066}
\DeclareTextGlyphY{LinLibertine_I}{afii10045}{1067}
\DeclareTextGlyphY{LinLibertine_I}{uni042B}{1067}
\DeclareTextGlyphY{LinLibertine_I}{afii10046}{1068}
\DeclareTextGlyphY{LinLibertine_I}{uni042C}{1068}
\DeclareTextGlyphY{LinLibertine_I}{afii10047}{1069}
\DeclareTextGlyphY{LinLibertine_I}{uni042D}{1069}
\DeclareTextGlyphY{LinLibertine_I}{afii10048}{1070}
\DeclareTextGlyphY{LinLibertine_I}{uni042E}{1070}
\DeclareTextGlyphY{LinLibertine_I}{afii10049}{1071}
\DeclareTextGlyphY{LinLibertine_I}{uni042F}{1071}
\DeclareTextGlyphY{LinLibertine_I}{uni05C6}{1478}
\DeclareTextGlyphY{LinLibertine_I}{afii57664}{1488}
\DeclareTextGlyphY{LinLibertine_I}{uni05D0}{1488}
\DeclareTextGlyphY{LinLibertine_I}{afii57665}{1489}
\DeclareTextGlyphY{LinLibertine_I}{uni05D1}{1489}
\DeclareTextGlyphY{LinLibertine_I}{afii57666}{1490}
\DeclareTextGlyphY{LinLibertine_I}{uni05D2}{1490}
\DeclareTextGlyphY{LinLibertine_I}{afii57667}{1491}
\DeclareTextGlyphY{LinLibertine_I}{uni05D3}{1491}
\DeclareTextGlyphY{LinLibertine_I}{afii57668}{1492}
\DeclareTextGlyphY{LinLibertine_I}{uni05D4}{1492}
\DeclareTextGlyphY{LinLibertine_I}{afii57669}{1493}
\DeclareTextGlyphY{LinLibertine_I}{uni05D5}{1493}
\DeclareTextGlyphY{LinLibertine_I}{afii57670}{1494}
\DeclareTextGlyphY{LinLibertine_I}{uni05D6}{1494}
\DeclareTextGlyphY{LinLibertine_I}{afii57671}{1495}
\DeclareTextGlyphY{LinLibertine_I}{uni05D7}{1495}
\DeclareTextGlyphY{LinLibertine_I}{afii57672}{1496}
\DeclareTextGlyphY{LinLibertine_I}{uni05D8}{1496}
\DeclareTextGlyphY{LinLibertine_I}{afii57673}{1497}
\DeclareTextGlyphY{LinLibertine_I}{uni05D9}{1497}
\DeclareTextGlyphY{LinLibertine_I}{afii57674}{1498}
\DeclareTextGlyphY{LinLibertine_I}{uni05DA}{1498}
\DeclareTextGlyphY{LinLibertine_I}{afii57675}{1499}
\DeclareTextGlyphY{LinLibertine_I}{uni05DB}{1499}
\DeclareTextGlyphY{LinLibertine_I}{afii57676}{1500}
\DeclareTextGlyphY{LinLibertine_I}{uni05DC}{1500}
\DeclareTextGlyphY{LinLibertine_I}{afii57677}{1501}
\DeclareTextGlyphY{LinLibertine_I}{uni05DD}{1501}
\DeclareTextGlyphY{LinLibertine_I}{afii57678}{1502}
\DeclareTextGlyphY{LinLibertine_I}{uni05DE}{1502}
\DeclareTextGlyphY{LinLibertine_I}{afii57679}{1503}
\DeclareTextGlyphY{LinLibertine_I}{uni05DF}{1503}
\DeclareTextGlyphY{LinLibertine_I}{afii57680}{1504}
\DeclareTextGlyphY{LinLibertine_I}{uni05E0}{1504}
\DeclareTextGlyphY{LinLibertine_I}{afii57681}{1505}
\DeclareTextGlyphY{LinLibertine_I}{uni05E1}{1505}
\DeclareTextGlyphY{LinLibertine_I}{afii57682}{1506}
\DeclareTextGlyphY{LinLibertine_I}{uni05E2}{1506}
\DeclareTextGlyphY{LinLibertine_I}{afii57683}{1507}
\DeclareTextGlyphY{LinLibertine_I}{uni05E3}{1507}
\DeclareTextGlyphY{LinLibertine_I}{afii57684}{1508}
\DeclareTextGlyphY{LinLibertine_I}{uni05E4}{1508}
\DeclareTextGlyphY{LinLibertine_I}{afii57685}{1509}
\DeclareTextGlyphY{LinLibertine_I}{uni05E5}{1509}
\DeclareTextGlyphY{LinLibertine_I}{afii57686}{1510}
\DeclareTextGlyphY{LinLibertine_I}{uni05E6}{1510}
\DeclareTextGlyphY{LinLibertine_I}{afii57687}{1511}
\DeclareTextGlyphY{LinLibertine_I}{uni05E7}{1511}
\DeclareTextGlyphY{LinLibertine_I}{afii57688}{1512}
\DeclareTextGlyphY{LinLibertine_I}{uni05E8}{1512}
\DeclareTextGlyphY{LinLibertine_I}{afii57689}{1513}
\DeclareTextGlyphY{LinLibertine_I}{uni05E9}{1513}
\DeclareTextGlyphY{LinLibertine_I}{afii57690}{1514}
\DeclareTextGlyphY{LinLibertine_I}{uni05EA}{1514}
\DeclareTextGlyphY{LinLibertine_I}{afii57716}{1520}
\DeclareTextGlyphY{LinLibertine_I}{uni05F0}{1520}
\DeclareTextGlyphY{LinLibertine_I}{afii57717}{1521}
\DeclareTextGlyphY{LinLibertine_I}{uni05F1}{1521}
\DeclareTextGlyphY{LinLibertine_I}{afii57718}{1522}
\DeclareTextGlyphY{LinLibertine_I}{uni05F2}{1522}
\DeclareTextGlyphY{LinLibertine_I}{uni05F3}{1523}
\DeclareTextGlyphY{LinLibertine_I}{uni05F4}{1524}
\DeclareTextGlyphY{LinLibertine_I}{Germandbls}{7838}
\DeclareTextGlyphY{LinLibertine_I}{uni1E9E}{7838}
\DeclareTextGlyphY{LinLibertine_I}{Oneroman}{8544}
\DeclareTextGlyphY{LinLibertine_I}{uni2160}{8544}
\DeclareTextGlyphY{LinLibertine_I}{Tworoman}{8545}
\DeclareTextGlyphY{LinLibertine_I}{uni2161}{8545}
\DeclareTextGlyphY{LinLibertine_I}{Threeroman}{8546}
\DeclareTextGlyphY{LinLibertine_I}{uni2162}{8546}
\DeclareTextGlyphY{LinLibertine_I}{Fourroman}{8547}
\DeclareTextGlyphY{LinLibertine_I}{uni2163}{8547}
\DeclareTextGlyphY{LinLibertine_I}{Fiveroman}{8548}
\DeclareTextGlyphY{LinLibertine_I}{uni2164}{8548}
\DeclareTextGlyphY{LinLibertine_I}{Sixroman}{8549}
\DeclareTextGlyphY{LinLibertine_I}{uni2165}{8549}
\DeclareTextGlyphY{LinLibertine_I}{Sevenroman}{8550}
\DeclareTextGlyphY{LinLibertine_I}{uni2166}{8550}
\DeclareTextGlyphY{LinLibertine_I}{Eightroman}{8551}
\DeclareTextGlyphY{LinLibertine_I}{uni2167}{8551}
\DeclareTextGlyphY{LinLibertine_I}{Nineroman}{8552}
\DeclareTextGlyphY{LinLibertine_I}{uni2168}{8552}
\DeclareTextGlyphY{LinLibertine_I}{Tenroman}{8553}
\DeclareTextGlyphY{LinLibertine_I}{uni2169}{8553}
\DeclareTextGlyphY{LinLibertine_I}{Elevenroman}{8554}
\DeclareTextGlyphY{LinLibertine_I}{uni216A}{8554}
\DeclareTextGlyphY{LinLibertine_I}{Twelveroman}{8555}
\DeclareTextGlyphY{LinLibertine_I}{uni216B}{8555}
\DeclareTextGlyphY{LinLibertine_I}{uni216C}{8556}
\DeclareTextGlyphY{LinLibertine_I}{uni216D}{8557}
\DeclareTextGlyphY{LinLibertine_I}{uni216E}{8558}
\DeclareTextGlyphY{LinLibertine_I}{uni216F}{8559}
\DeclareTextGlyphY{LinLibertine_I}{uni24B6}{9398}
\DeclareTextGlyphY{LinLibertine_I}{uni24B7}{9399}
\DeclareTextGlyphY{LinLibertine_I}{uni24B8}{9400}
\DeclareTextGlyphY{LinLibertine_I}{uni24B9}{9401}
\DeclareTextGlyphY{LinLibertine_I}{uni24BA}{9402}
\DeclareTextGlyphY{LinLibertine_I}{uni24BB}{9403}
\DeclareTextGlyphY{LinLibertine_I}{uni24BC}{9404}
\DeclareTextGlyphY{LinLibertine_I}{uni24BE}{9406}
\DeclareTextGlyphY{LinLibertine_I}{uni24BF}{9407}
\DeclareTextGlyphY{LinLibertine_I}{uni24C0}{9408}
\DeclareTextGlyphY{LinLibertine_I}{uni24C1}{9409}
\DeclareTextGlyphY{LinLibertine_I}{uni24C2}{9410}
\DeclareTextGlyphY{LinLibertine_I}{uni24C3}{9411}
\DeclareTextGlyphY{LinLibertine_I}{uni24C4}{9412}
\DeclareTextGlyphY{LinLibertine_I}{uni24C5}{9413}
\DeclareTextGlyphY{LinLibertine_I}{uni24C6}{9414}
\DeclareTextGlyphY{LinLibertine_I}{uni24C7}{9415}
\DeclareTextGlyphY{LinLibertine_I}{uni24C8}{9416}
\DeclareTextGlyphY{LinLibertine_I}{uni24CA}{9418}
\DeclareTextGlyphY{LinLibertine_I}{uni24CB}{9419}
\DeclareTextGlyphY{LinLibertine_I}{uni24CC}{9420}
\DeclareTextGlyphY{LinLibertine_I}{uni24CD}{9421}
\DeclareTextGlyphY{LinLibertine_I}{uni24CE}{9422}
\DeclareTextGlyphY{LinLibertine_I}{uni24CF}{9423}
\DeclareTextGlyphY{LinLibertine_I}{Tux}{57344}
\DeclareTextGlyphY{LinLibertine_I}{uniE000}{57344}
\DeclareTextGlyphY{LinLibertine_I}{uniE001}{57345}
\DeclareTextGlyphY{LinLibertine_I}{uniE002}{57346}
\DeclareTextGlyphY{LinLibertine_I}{uniE003}{57347}
\DeclareTextGlyphY{LinLibertine_I}{uniE004}{57348}
\DeclareTextGlyphY{LinLibertine_I}{uniE005}{57349}
\DeclareTextGlyphY{LinLibertine_I}{uniE006}{57350}
\DeclareTextGlyphY{LinLibertine_I}{uniE007}{57351}
\DeclareTextGlyphY{LinLibertine_I}{uniE008}{57352}
\DeclareTextGlyphY{LinLibertine_I}{uniE009}{57353}
\DeclareTextGlyphY{LinLibertine_I}{uniE00A}{57354}
\DeclareTextGlyphY{LinLibertine_I}{uniE00B}{57355}
\DeclareTextGlyphY{LinLibertine_I}{copyleft}{57356}
\DeclareTextGlyphY{LinLibertine_I}{uniE00C}{57356}
\DeclareTextGlyphY{LinLibertine_I}{publicdomain}{57357}
\DeclareTextGlyphY{LinLibertine_I}{uniE00D}{57357}
\DeclareTextGlyphY{LinLibertine_I}{creativecommons}{57358}
\DeclareTextGlyphY{LinLibertine_I}{uniE00E}{57358}
\DeclareTextGlyphY{LinLibertine_I}{zero.fitted}{57360}
\DeclareTextGlyphY{LinLibertine_I}{uniE010}{57360}
\DeclareTextGlyphY{LinLibertine_I}{one.fitted}{57361}
\DeclareTextGlyphY{LinLibertine_I}{uniE011}{57361}
\DeclareTextGlyphY{LinLibertine_I}{two.fitted}{57362}
\DeclareTextGlyphY{LinLibertine_I}{uniE012}{57362}
\DeclareTextGlyphY{LinLibertine_I}{three.fitted}{57363}
\DeclareTextGlyphY{LinLibertine_I}{uniE013}{57363}
\DeclareTextGlyphY{LinLibertine_I}{four.fitted}{57364}
\DeclareTextGlyphY{LinLibertine_I}{uniE014}{57364}
\DeclareTextGlyphY{LinLibertine_I}{five.fitted}{57365}
\DeclareTextGlyphY{LinLibertine_I}{uniE015}{57365}
\DeclareTextGlyphY{LinLibertine_I}{six.fitted}{57366}
\DeclareTextGlyphY{LinLibertine_I}{uniE016}{57366}
\DeclareTextGlyphY{LinLibertine_I}{seven.fitted}{57367}
\DeclareTextGlyphY{LinLibertine_I}{uniE017}{57367}
\DeclareTextGlyphY{LinLibertine_I}{eight.fitted}{57368}
\DeclareTextGlyphY{LinLibertine_I}{uniE018}{57368}
\DeclareTextGlyphY{LinLibertine_I}{nine.fitted}{57369}
\DeclareTextGlyphY{LinLibertine_I}{uniE019}{57369}
\DeclareTextGlyphY{LinLibertine_I}{W.alt}{57391}
\DeclareTextGlyphY{LinLibertine_I}{uniE02F}{57391}
\DeclareTextGlyphY{LinLibertine_I}{uniE040}{57408}
\DeclareTextGlyphY{LinLibertine_I}{uniE041}{57409}
\DeclareTextGlyphY{LinLibertine_I}{uniE042}{57410}
\DeclareTextGlyphY{LinLibertine_I}{ampersand.alt}{57424}
\DeclareTextGlyphY{LinLibertine_I}{uniE050}{57424}
\DeclareTextGlyphY{LinLibertine_I}{a.sc}{57425}
\DeclareTextGlyphY{LinLibertine_I}{uniE051}{57425}
\DeclareTextGlyphY{LinLibertine_I}{b.sc}{57426}
\DeclareTextGlyphY{LinLibertine_I}{uniE052}{57426}
\DeclareTextGlyphY{LinLibertine_I}{c.sc}{57427}
\DeclareTextGlyphY{LinLibertine_I}{uniE053}{57427}
\DeclareTextGlyphY{LinLibertine_I}{d.sc}{57428}
\DeclareTextGlyphY{LinLibertine_I}{uniE054}{57428}
\DeclareTextGlyphY{LinLibertine_I}{e.sc}{57429}
\DeclareTextGlyphY{LinLibertine_I}{uniE055}{57429}
\DeclareTextGlyphY{LinLibertine_I}{f.sc}{57430}
\DeclareTextGlyphY{LinLibertine_I}{uniE056}{57430}
\DeclareTextGlyphY{LinLibertine_I}{g.sc}{57431}
\DeclareTextGlyphY{LinLibertine_I}{uniE057}{57431}
\DeclareTextGlyphY{LinLibertine_I}{h.sc}{57432}
\DeclareTextGlyphY{LinLibertine_I}{uniE058}{57432}
\DeclareTextGlyphY{LinLibertine_I}{i.sc}{57433}
\DeclareTextGlyphY{LinLibertine_I}{uniE059}{57433}
\DeclareTextGlyphY{LinLibertine_I}{j.sc}{57434}
\DeclareTextGlyphY{LinLibertine_I}{uniE05A}{57434}
\DeclareTextGlyphY{LinLibertine_I}{k.sc}{57435}
\DeclareTextGlyphY{LinLibertine_I}{uniE05B}{57435}
\DeclareTextGlyphY{LinLibertine_I}{l.sc}{57436}
\DeclareTextGlyphY{LinLibertine_I}{uniE05C}{57436}
\DeclareTextGlyphY{LinLibertine_I}{m.sc}{57437}
\DeclareTextGlyphY{LinLibertine_I}{uniE05D}{57437}
\DeclareTextGlyphY{LinLibertine_I}{n.sc}{57438}
\DeclareTextGlyphY{LinLibertine_I}{uniE05E}{57438}
\DeclareTextGlyphY{LinLibertine_I}{o.sc}{57439}
\DeclareTextGlyphY{LinLibertine_I}{uniE05F}{57439}
\DeclareTextGlyphY{LinLibertine_I}{p.sc}{57440}
\DeclareTextGlyphY{LinLibertine_I}{uniE060}{57440}
\DeclareTextGlyphY{LinLibertine_I}{q.sc}{57441}
\DeclareTextGlyphY{LinLibertine_I}{uniE061}{57441}
\DeclareTextGlyphY{LinLibertine_I}{r.sc}{57442}
\DeclareTextGlyphY{LinLibertine_I}{uniE062}{57442}
\DeclareTextGlyphY{LinLibertine_I}{s.sc}{57443}
\DeclareTextGlyphY{LinLibertine_I}{uniE063}{57443}
\DeclareTextGlyphY{LinLibertine_I}{t.sc}{57444}
\DeclareTextGlyphY{LinLibertine_I}{uniE064}{57444}
\DeclareTextGlyphY{LinLibertine_I}{u.sc}{57445}
\DeclareTextGlyphY{LinLibertine_I}{uniE065}{57445}
\DeclareTextGlyphY{LinLibertine_I}{v.sc}{57446}
\DeclareTextGlyphY{LinLibertine_I}{uniE066}{57446}
\DeclareTextGlyphY{LinLibertine_I}{w.sc}{57447}
\DeclareTextGlyphY{LinLibertine_I}{uniE067}{57447}
\DeclareTextGlyphY{LinLibertine_I}{x.sc}{57448}
\DeclareTextGlyphY{LinLibertine_I}{uniE068}{57448}
\DeclareTextGlyphY{LinLibertine_I}{y.sc}{57449}
\DeclareTextGlyphY{LinLibertine_I}{uniE069}{57449}
\DeclareTextGlyphY{LinLibertine_I}{z.sc}{57450}
\DeclareTextGlyphY{LinLibertine_I}{uniE06A}{57450}
\DeclareTextGlyphY{LinLibertine_I}{uniE06B}{57451}
\DeclareTextGlyphY{LinLibertine_I}{hyphen.sc}{57453}
\DeclareTextGlyphY{LinLibertine_I}{uniE06D}{57453}
\DeclareTextGlyphY{LinLibertine_I}{adieresis.sc}{57460}
\DeclareTextGlyphY{LinLibertine_I}{uniE074}{57460}
\DeclareTextGlyphY{LinLibertine_I}{ae.sc}{57462}
\DeclareTextGlyphY{LinLibertine_I}{uniE076}{57462}
\DeclareTextGlyphY{LinLibertine_I}{odieresis.sc}{57478}
\DeclareTextGlyphY{LinLibertine_I}{uniE086}{57478}
\DeclareTextGlyphY{LinLibertine_I}{oe.sc}{57479}
\DeclareTextGlyphY{LinLibertine_I}{uniE087}{57479}
\DeclareTextGlyphY{LinLibertine_I}{thorn.sc}{57486}
\DeclareTextGlyphY{LinLibertine_I}{uniE08E}{57486}
\DeclareTextGlyphY{LinLibertine_I}{ij.sc}{57488}
\DeclareTextGlyphY{LinLibertine_I}{uniE090}{57488}
\DeclareTextGlyphY{LinLibertine_I}{germandbls.sc}{57490}
\DeclareTextGlyphY{LinLibertine_I}{uniE092}{57490}
\DeclareTextGlyphY{LinLibertine_I}{Q_u.sc}{57491}
\DeclareTextGlyphY{LinLibertine_I}{uniE093}{57491}
\DeclareTextGlyphY{LinLibertine_I}{eng.sc}{57508}
\DeclareTextGlyphY{LinLibertine_I}{uniE0A4}{57508}
\DeclareTextGlyphY{LinLibertine_I}{ohungarumlaut.sc}{57509}
\DeclareTextGlyphY{LinLibertine_I}{uniE0A5}{57509}
\DeclareTextGlyphY{LinLibertine_I}{uhungarumlaut.sc}{57518}
\DeclareTextGlyphY{LinLibertine_I}{uniE0AE}{57518}
\DeclareTextGlyphY{LinLibertine_I}{uniE104}{57604}
\DeclareTextGlyphY{LinLibertine_I}{uniE105}{57605}
\DeclareTextGlyphY{LinLibertine_I}{uniE106}{57606}
\DeclareTextGlyphY{LinLibertine_I}{uniE107}{57607}
\DeclareTextGlyphY{LinLibertine_I}{leaf}{57656}
\DeclareTextGlyphY{LinLibertine_I}{uniE138}{57656}
\DeclareTextGlyphY{LinLibertine_I}{hungarumlaut.cap}{58205}
\DeclareTextGlyphY{LinLibertine_I}{uniE35D}{58205}
\DeclareTextGlyphY{LinLibertine_I}{breve.cyrcap}{58208}
\DeclareTextGlyphY{LinLibertine_I}{uniE360}{58208}
\DeclareTextGlyphY{LinLibertine_I}{breve.cyr}{58209}
\DeclareTextGlyphY{LinLibertine_I}{uniE361}{58209}
\DeclareTextGlyphY{LinLibertine_I}{dieresis.cap}{58210}
\DeclareTextGlyphY{LinLibertine_I}{uniE362}{58210}
\DeclareTextGlyphY{LinLibertine_I}{metric}{58400}
\DeclareTextGlyphY{LinLibertine_I}{uniE420}{58400}
\DeclareTextGlyphY{LinLibertine_I}{uniFFFD}{65533}


==> binhex.tex <==
%%
%% This is file `binhex.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% binhex.dtx  (with options: `style')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from binhex.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file binhex.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
\edef\next{\toks0=%
   {\catcode`\noexpand\@=\the\catcode`\@\toks0{\the\toks0}}%
}
\next
\catcode`\@11
\def\next#1#2#3{\expandafter \def \csname bb@#1\endcsname##1%
  {#2\csname bb@#3##1\endcsname}}
\next{00}00 \next{01}01 \next{02}10 \next{03}11
\next{04}20 \next{05}21 \next{06}30 \next{07}31
\next{08}40 \next{09}41 \next{10}50 \next{11}51
\next{12}60 \next{13}61 \next{14}70 \next{15}71
\next{16}80 \next{17}81 \next{18}90 \next{19}91
\expandafter \def \csname bb@0+\endcsname {+0}
\expandafter \def \csname bb@1+\endcsname {+1}
\def\bb@endbinary#1+{\fi\fi}
\expandafter \def \csname bb@0-\endcsname {0+-\bb@dobinary}
\expandafter\def\csname bb@0m\endcsname#1+{#1+0}
\expandafter\def\csname bb@1m\endcsname#1+{#1+1}
\def\bb@dobinary#1#2{\if#10\if m\string#2\else\bb@endbinary\fi\fi
 \expandafter\bb@dobinary\number\csname bb@0#1\endcsname#2}
\def\nbinary#1#2{\expandafter\bb@dobinary\number\number#2%
 \romannumeral\number\number#1 000+}
\def\binary{\nbinary1}
\def \next #1#2{\expandafter \def
 \csname bb@h\number +#1\endcsname ##1+{\bb@dohex ##1+#2}%
}
\next   {0}0 \next   {1}1 \next  {10}2 \next  {11}3
\next {100}4 \next {101}5 \next {110}6 \next {111}7
\next{1000}8 \next{1001}9 \next{1010}A \next{1011}B
\next{1100}C \next{1101}D \next{1110}E \next{1111}F
\def\bb@dohex #1{\csname bb@x#1\endcsname}
\def\bb@x\endcsname#1{ \bb@xm{m\endcsname}}
\def\bb@xm #1\endcsname #2#3+{#2#3%
 \csname bb@h\number+\endcsname
 #1\endcsname m#3+}
\def\bb@nbinbased #1#2#3{\expandafter \bb@dobinary \number#1%
 \expandafter \bb@dohex
 \romannumeral \number\number #2 000\expandafter\endcsname
 \romannumeral \number\number #3 000+}
\def\nbinbased #1#2#3{\expandafter\bb@nbinbased
 \expandafter {\number#3}{#2}{#1}}
\def\nhex{\nbinbased4}
\def\noct{\nbinbased3}
\def\ntetra{\nbinbased2}
\def\hex{\nhex1}
\def\oct{\noct1}
\def\tetra{\ntetra1}
\the\toks0
\endinput
%%
%% End of file `binhex.tex'.


==> keyval.tex <==
%%
%% This is file `keyval.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xkeyval.dtx  (with options: `xkvkeyval')
%% 
%% ---------------------------------------
%% Copyright (C) 2004-2014 Hendri Adriaens
%% ---------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2003/12/01 or later.
%%
%% This work has the LPPL maintenance status "maintained".
%%
%% This Current Maintainer of this work is Hendri Adriaens.
%%
%% This work consists of the file xkeyval.dtx and derived files
%% keyval.tex, xkvtxhdr.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvutils.tex, pst-xkey.tex, pst-xkey.sty, xkveca.cls,
%% xkvecb.cls, xkvesa.sty, xkvesb.sty, xkvesc.sty, xkvex1.tex,
%% xkvex2.tex, xkvex3.tex and xkvex4.tex.
%%
%% The following files constitute the xkeyval bundle and must be
%% distributed as a whole: readme, xkeyval.pdf, keyval.tex,
%% pst-xkey.sty, pst-xkey.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvtxhdr.tex, xkvutils.tex, pst-xkey.dtx and xkeyval.dtx.
%%
%%
%% Based on keyval.sty.
%%
\def\XKV@tempa#1{%
\long\def\KV@@sp@def##1##2{%
  \futurelet\XKV@resa\KV@@sp@d##2\@nil\@nil#1\@nil\relax##1}%
\long\def\KV@@sp@d{%
  \ifx\XKV@resa\@sptoken
    \expandafter\KV@@sp@b
  \else
    \expandafter\KV@@sp@b\expandafter#1%
  \fi}%
\long\def\KV@@sp@b#1##1 \@nil{\KV@@sp@c##1}%
  }
\XKV@tempa{ }
\long\def\KV@@sp@c#1\@nil#2\relax#3{\XKV@toks{#1}\edef#3{\the\XKV@toks}}
\long\def\KV@do#1,{%
 \ifx\relax#1\@empty\else
  \KV@split#1==\relax
  \expandafter\KV@do\fi}
\long\def\KV@split#1=#2=#3\relax{%
  \KV@@sp@def\XKV@tempa{#1}%
  \ifx\XKV@tempa\@empty\else
    \expandafter\let\expandafter\XKV@tempc
      \csname\KV@prefix\XKV@tempa\endcsname
    \ifx\XKV@tempc\relax
      \XKV@err{`\XKV@tempa' undefined}%
    \else
      \ifx\@empty#3\@empty
        \KV@default
      \else
        \KV@@sp@def\XKV@tempb{#2}%
        \expandafter\XKV@tempc\expandafter{\XKV@tempb}\relax
      \fi
    \fi
  \fi}
\def\KV@default{%
  \expandafter\let\expandafter\XKV@tempb
    \csname\KV@prefix\XKV@tempa @default\endcsname
  \ifx\XKV@tempb\relax
    \XKV@err{No value specified for key `\XKV@tempa'}%
  \else
    \XKV@tempb\relax
  \fi}
\def\KV@def#1#2[#3]{%
  \long\@namedef{KV@#1@#2@default\expandafter}\expandafter
    {\csname KV@#1@#2\endcsname{#3}}%
  \long\@namedef{KV@#1@#2}##1}
\endinput
%%
%% End of file `keyval.tex'.


==> xkeyval.tex <==
%%
%% This is file `xkeyval.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xkeyval.dtx  (with options: `xkvtex')
%% 
%% ---------------------------------------
%% Copyright (C) 2004-2014 Hendri Adriaens
%% ---------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2003/12/01 or later.
%%
%% This work has the LPPL maintenance status "maintained".
%%
%% This Current Maintainer of this work is Hendri Adriaens.
%%
%% This work consists of the file xkeyval.dtx and derived files
%% keyval.tex, xkvtxhdr.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvutils.tex, pst-xkey.tex, pst-xkey.sty, xkveca.cls,
%% xkvecb.cls, xkvesa.sty, xkvesb.sty, xkvesc.sty, xkvex1.tex,
%% xkvex2.tex, xkvex3.tex and xkvex4.tex.
%%
%% The following files constitute the xkeyval bundle and must be
%% distributed as a whole: readme, xkeyval.pdf, keyval.tex,
%% pst-xkey.sty, pst-xkey.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvtxhdr.tex, xkvutils.tex, pst-xkey.dtx and xkeyval.dtx.
%%
\csname XKeyValLoaded\endcsname
\let\XKeyValLoaded\endinput
\edef\XKVcatcodes{%
  \catcode`\noexpand\@\the\catcode`\@\relax
  \catcode`\noexpand\=\the\catcode`\=\relax
  \catcode`\noexpand\,\the\catcode`\,\relax
  \catcode`\noexpand\:\the\catcode`\:\relax
  \let\noexpand\XKVcatcodes\relax
}
\catcode`\@11\relax
\catcode`\=12\relax
\catcode`\,12\relax
\catcode`\:12\relax
\input xkvutils
\newcount\XKV@depth
\newif\ifXKV@st
\newif\ifXKV@sg
\newif\ifXKV@pl
\newif\ifXKV@knf
\newif\ifXKV@rkv
\newif\ifXKV@inpox
\newif\ifXKV@preset
\let\XKV@rm\@empty
\ifx\ProvidesFile\@undefined
  \message{2014/12/03 v2.7a key=value parser (HA)}
  \input xkvtxhdr
\else
  \ProvidesFile{xkeyval.tex}[2014/12/03 v2.7a key=value parser (HA)]
  \@addtofilelist{xkeyval.tex}
\fi
\def\XKV@warn#1{\message{xkeyval warning: #1}}
\def\XKV@err#1{\errmessage{xkeyval error: #1}}
\def\KV@errx{\XKV@err}
\let\KV@err\KV@errx
\def\XKV@ifstar#1{\@ifnextcharacter*{\@firstoftwo{#1}}}
\def\XKV@ifplus#1{\@ifnextcharacter+{\@firstoftwo{#1}}}
\def\XKV@makepf#1{%
  \KV@@sp@def\XKV@prefix{#1}%
  \def\XKV@resa{XKV}%
  \ifx\XKV@prefix\XKV@resa
    \XKV@err{`XKV' prefix is not allowed}%
    \let\XKV@prefix\@empty
  \else
    \edef\XKV@prefix{\ifx\XKV@prefix\@empty\else\XKV@prefix @\fi}%
  \fi
}
\def\XKV@makehd#1{%
  \expandafter\KV@@sp@def\expandafter\XKV@header\expandafter{#1}%
  \edef\XKV@header{%
    \XKV@prefix\ifx\XKV@header\@empty\else\XKV@header @\fi
  }%
}
\def\XKV@srstate#1#2{%
  \ifx\@empty#2\@empty\advance\XKV@depth\@ne\fi
  \XKV@for@n{XKV@prefix,XKV@fams,XKV@tkey,XKV@na,%
    ifXKV@st,ifXKV@pl,ifXKV@knf,CurrentOption}\XKV@resa{%
    \expandafter\let\csname\XKV@resa#1\expandafter
      \endcsname\csname\XKV@resa#2\endcsname
  }%
  \ifx\@empty#1\@empty\advance\XKV@depth\m@ne\fi
}
\def\XKV@testopta#1{%
  \XKV@ifstar{\XKV@sttrue\XKV@t@stopta{#1}}%
    {\XKV@stfalse\XKV@t@stopta{#1}}%
}
\def\XKV@t@stopta#1{\XKV@ifplus{\XKV@pltrue#1}{\XKV@plfalse#1}}
\def\XKV@testoptb#1{\@testopt{\XKV@t@stoptb#1}{KV}}
\def\XKV@t@stoptb#1[#2]#3{%
  \XKV@makepf{#2}%
  \XKV@makehd{#3}%
  \KV@@sp@def\XKV@tfam{#3}%
  #1%
}
\def\XKV@testoptc#1{\@testopt{\XKV@t@stoptc#1}{KV}}
\def\XKV@t@stoptc#1[#2]#3{%
  \XKV@makepf{#2}%
  \XKV@checksanitizeb{#3}\XKV@fams
  \expandafter\XKV@sp@deflist\expandafter
    \XKV@fams\expandafter{\XKV@fams}%
  \@testopt#1{}%
}
\def\XKV@testoptd#1#2{%
  \XKV@testoptb{%
    \edef\XKV@tempa{#2\XKV@header}%
    \def\XKV@tempb{\@testopt{\XKV@t@stoptd#1}}%
    \expandafter\XKV@tempb\expandafter{\XKV@tempa}%
  }%
}
\def\XKV@t@stoptd#1[#2]#3{%
  \@ifnextchar[{\XKV@sttrue#1{#2}{#3}}{\XKV@stfalse#1{#2}{#3}[]}%
}
\def\XKV@ifcmd#1#2#3{%
  \def\XKV@@ifcmd##1#2##2##3\@nil##4{%
    \def##4{##2}\ifx##4\@nnil
      \def##4{##1}\expandafter\@secondoftwo
    \else
      \expandafter\@firstoftwo
    \fi
  }%
  \XKV@@ifcmd#1#2{\@nil}\@nil#3%
}
\def\XKV@getkeyname#1#2{\expandafter\XKV@g@tkeyname#1=\@nil#2}
\long\def\XKV@g@tkeyname#1=#2\@nil#3{%
  \XKV@ifcmd{#1}\savevalue#3{\XKV@rkvtrue\XKV@sgfalse}{%
    \XKV@ifcmd{#1}\gsavevalue#3%
      {\XKV@rkvtrue\XKV@sgtrue}{\XKV@rkvfalse\XKV@sgfalse}%
  }%
}
\def\XKV@getsg#1#2{%
  \expandafter\XKV@ifcmd\expandafter{#1}\global#2\XKV@sgtrue\XKV@sgfalse
}
\def\XKV@define@default#1#2{%
  \expandafter\def\csname\XKV@header#1@default\expandafter
    \endcsname\expandafter{\csname\XKV@header#1\endcsname{#2}}%
}
\def\define@key{\XKV@testoptb\XKV@define@key}
\def\XKV@define@key#1{%
  \@ifnextchar[{\XKV@d@fine@k@y{#1}}{%
    \long\expandafter\def\csname\XKV@header#1\endcsname####1%
  }%
}
\def\XKV@d@fine@k@y#1[#2]{%
  \XKV@define@default{#1}{#2}%
  \expandafter\def\csname\XKV@header#1\endcsname##1%
}
\def\define@cmdkey{\XKV@testoptd\XKV@define@cmdkey{cmd}}
\def\XKV@define@cmdkey#1#2[#3]#4{%
  \ifXKV@st\XKV@define@default{#2}{#3}\fi
  \def\XKV@tempa{\expandafter\def\csname\XKV@header#2\endcsname####1}%
  \begingroup\expandafter\endgroup\expandafter\XKV@tempa\expandafter
    {\expandafter\def\csname#1#2\endcsname{##1}#4}%
}
\def\define@cmdkeys{\XKV@testoptd\XKV@define@cmdkeys{cmd}}
\def\XKV@define@cmdkeys#1#2[#3]{%
  \XKV@sp@deflist\XKV@tempa{#2}%
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \edef\XKV@tempa{\noexpand\XKV@define@cmdkey{#1}{\XKV@tempa}}%
    \XKV@tempa[#3]{}%
  }%
}
\def\define@choicekey{\XKV@testopta{\XKV@testoptb\XKV@define@choicekey}}
\def\XKV@define@choicekey#1{\@testopt{\XKV@d@fine@choicekey{#1}}{}}
\def\XKV@d@fine@choicekey#1[#2]#3{%
  \toks@{#2}%
  \XKV@sp@deflist\XKV@tempa{#3}\XKV@toks\expandafter{\XKV@tempa}%
  \@ifnextchar[{\XKV@d@fine@ch@icekey{#1}}{\XKV@d@fine@ch@ic@key{#1}}%
}
\def\XKV@d@fine@ch@icekey#1[#2]{%
  \XKV@define@default{#1}{#2}%
  \XKV@d@fine@ch@ic@key{#1}%
}
\def\XKV@d@fine@ch@ic@key#1{%
  \ifXKV@pl\XKV@afterelsefi
    \expandafter\XKV@d@f@ne@ch@ic@k@y
  \else\XKV@afterfi
    \expandafter\XKV@d@f@ne@ch@ic@key
  \fi
  \csname\XKV@header#1\endcsname
}
\def\XKV@d@f@ne@ch@ic@key#1#2{\XKV@d@f@n@@ch@ic@k@y#1{{#2}}}
\def\XKV@d@f@ne@ch@ic@k@y#1#2#3{\XKV@d@f@n@@ch@ic@k@y#1{{#2}{#3}}}
\def\XKV@d@f@n@@ch@ic@k@y#1#2{%
  \edef#1##1{%
    \ifXKV@st\noexpand\XKV@sttrue\else\noexpand\XKV@stfalse\fi
    \ifXKV@pl\noexpand\XKV@pltrue\else\noexpand\XKV@plfalse\fi
    \noexpand\XKV@checkchoice[\the\toks@]{##1}{\the\XKV@toks}%
  }%
  \def\XKV@tempa{\def#1####1}%
  \expandafter\XKV@tempa\expandafter{#1{##1}#2}%
}
\def\define@boolkey{\XKV@t@stopta{\XKV@testoptd\XKV@define@boolkey{}}}
\def\XKV@define@boolkey#1#2[#3]{%
  \ifXKV@pl\XKV@afterelsefi
    \expandafter\XKV@d@f@ne@boolkey
  \else\XKV@afterfi
    \expandafter\XKV@d@fine@boolkey
  \fi
  \csname\XKV@header#2\endcsname{#2}{#1#2}{#3}%
}
\def\XKV@d@fine@boolkey#1#2#3#4#5{%
  \XKV@d@f@ne@b@olkey#1{#2}{#3}{#4}%
    {{\csname#3\XKV@resa\endcsname#5}}%
}
\def\XKV@d@f@ne@boolkey#1#2#3#4#5#6{%
  \XKV@d@f@ne@b@olkey#1{#2}{#3}{#4}%
    {{\csname#3\XKV@resa\endcsname#5}{#6}}%
}
\def\XKV@d@f@ne@b@olkey#1#2#3#4#5{%
  \expandafter\newif\csname if#3\endcsname
  \ifXKV@st\XKV@define@default{#2}{#4}\fi
  \ifXKV@pl
    \def#1##1{\XKV@pltrue\XKV@sttrue
      \XKV@checkchoice[\XKV@resa]{##1}{true,false}#5%
    }%
  \else
    \def#1##1{\XKV@plfalse\XKV@sttrue
      \XKV@checkchoice[\XKV@resa]{##1}{true,false}#5%
    }%
  \fi
}
\def\define@boolkeys{\XKV@plfalse\XKV@testoptd\XKV@define@boolkeys{}}
\def\XKV@define@boolkeys#1#2[#3]{%
  \XKV@sp@deflist\XKV@tempa{#2}%
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \expandafter\XKV@d@fine@boolkeys\expandafter{\XKV@tempa}{#1}{#3}%
  }%
}
\def\XKV@d@fine@boolkeys#1#2#3{%
  \expandafter\XKV@d@f@ne@b@olkey\csname\XKV@header#1\endcsname
    {#1}{#2#1}{#3}{{\csname#2#1\XKV@resa\endcsname}}%
}
\def\XKV@cc{\XKV@testopta{\@testopt\XKV@checkchoice{}}}
\def\XKV@checkchoice[#1]#2#3{%
  \def\XKV@tempa{#1}%
  \ifXKV@st\lowercase{\fi
  \ifx\XKV@tempa\@empty
    \def\XKV@tempa{\XKV@ch@ckch@ice\@nil{#2}{#3}}%
  \else
    \def\XKV@tempa{\XKV@ch@ckchoice#1\@nil{#2}{#3}}%
  \fi
  \ifXKV@st}\fi\XKV@tempa
}
\def\XKV@ch@ckchoice#1#2\@nil#3#4{%
  \def\XKV@tempa{#2}%
  \ifx\XKV@tempa\@empty\XKV@afterelsefi
    \XKV@ch@ckch@ice#1{#3}{#4}%
  \else\XKV@afterfi
    \XKV@@ch@ckchoice#1#2{#3}{#4}%
  \fi
}
\def\XKV@ch@ckch@ice#1#2#3{%
  \def\XKV@tempa{#1}%
  \ifx\XKV@tempa\@nnil\let\XKV@tempa\@empty\else
    \def\XKV@tempa{\def#1{#2}}%
  \fi
  \in@{,#2,}{,#3,}%
  \ifin@
    \ifXKV@pl
      \XKV@addtomacro@n\XKV@tempa\@firstoftwo
    \else
      \XKV@addtomacro@n\XKV@tempa\@firstofone
    \fi
  \else
    \ifXKV@pl
      \XKV@addtomacro@n\XKV@tempa\@secondoftwo
    \else
      \XKV@toks{#2}%
      \XKV@err{value `\the\XKV@toks' is not allowed}%
      \XKV@addtomacro@n\XKV@tempa\@gobble
    \fi
  \fi
  \XKV@tempa
}
\def\XKV@@ch@ckchoice#1#2#3#4{%
  \edef\XKV@tempa{\the\count@}\count@\z@
  \def\XKV@tempb{#3}%
  \def\XKV@tempc##1,{%
    \def#1{##1}%
    \ifx#1\@nnil
      \def#1{#3}\def#2{-1}\count@\XKV@tempa
      \ifXKV@pl
        \let\XKV@tempd\@secondoftwo
      \else
        \XKV@toks{#3}%
        \XKV@err{value `\the\XKV@toks' is not allowed}%
        \let\XKV@tempd\@gobble
      \fi
    \else
      \ifx#1\XKV@tempb
        \edef#2{\the\count@}\count@\XKV@tempa
        \ifXKV@pl
          \let\XKV@tempd\XKV@@ch@ckch@ice
        \else
          \let\XKV@tempd\XKV@@ch@ckch@ic@
        \fi
      \else
        \advance\count@\@ne
        \let\XKV@tempd\XKV@tempc
      \fi
    \fi
    \XKV@tempd
  }%
  \XKV@tempc#4,\@nil,%
}
\def\XKV@@ch@ckch@ice#1\@nil,{\@firstoftwo}
\def\XKV@@ch@ckch@ic@#1\@nil,{\@firstofone}
\def\key@ifundefined{\@testopt\XKV@key@ifundefined{KV}}
\def\XKV@key@ifundefined[#1]#2{%
  \XKV@makepf{#1}%
  \XKV@checksanitizeb{#2}\XKV@fams
  \expandafter\XKV@sp@deflist\expandafter
    \XKV@fams\expandafter{\XKV@fams}%
  \XKV@key@if@ndefined
}
\def\XKV@key@if@ndefined#1{%
  \XKV@knftrue
  \KV@@sp@def\XKV@tkey{#1}%
  \XKV@whilist\XKV@fams\XKV@tfam\ifXKV@knf\fi{%
    \XKV@makehd\XKV@tfam
    \XKV@ifundefined{\XKV@header\XKV@tkey}{}{\XKV@knffalse}%
  }%
  \ifXKV@knf
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
}
\def\disable@keys{\XKV@testoptb\XKV@disable@keys}
\def\XKV@disable@keys#1{%
  \XKV@checksanitizeb{#1}\XKV@tempa
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \XKV@ifundefined{\XKV@header\XKV@tempa}{%
      \XKV@err{key `\XKV@tempa' undefined}%
    }{%
      \edef\XKV@tempb{%
        \noexpand\XKV@warn{key `\XKV@tempa' has been disabled}%
      }%
      \XKV@ifundefined{\XKV@header\XKV@tempa @default}{%
        \edef\XKV@tempc{\noexpand\XKV@define@key{\XKV@tempa}}%
      }{%
        \edef\XKV@tempc{\noexpand\XKV@define@key{\XKV@tempa}[]}%
      }%
      \expandafter\XKV@tempc\expandafter{\XKV@tempb}%
    }%
  }%
}
\def\presetkeys{\XKV@stfalse\XKV@testoptb\XKV@presetkeys}
\def\gpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@presetkeys}
\def\XKV@presetkeys#1#2{%
  \XKV@pr@setkeys{#1}{preseth}%
  \XKV@pr@setkeys{#2}{presett}%
}
\def\XKV@pr@setkeys#1#2{%
  \XKV@ifundefined{XKV@\XKV@header#2}{%
    \XKV@checksanitizea{#1}\XKV@tempa
    \ifXKV@st\expandafter\global\fi\expandafter\def\csname
      XKV@\XKV@header#2\expandafter\endcsname\expandafter{\XKV@tempa}%
  }{%
    \expandafter\XKV@merge\csname XKV@\XKV@header
      #2\endcsname{#1}\XKV@getkeyname
  }%
}
\def\delpresetkeys{\XKV@stfalse\XKV@testoptb\XKV@delpresetkeys}
\def\gdelpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@delpresetkeys}
\def\XKV@delpresetkeys#1#2{%
  \XKV@d@lpresetkeys{#1}{preseth}%
  \XKV@d@lpresetkeys{#2}{presett}%
}
\def\XKV@d@lpresetkeys#1#2{%
  \XKV@ifundefined{XKV@\XKV@header#2}{%
    \XKV@err{no presets defined for `\XKV@header'}%
  }{%
    \expandafter\XKV@delete\csname XKV@\XKV@header
      #2\endcsname{#1}\XKV@getkeyname
  }%
}
\def\unpresetkeys{\XKV@stfalse\XKV@testoptb\XKV@unpresetkeys}
\def\gunpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@unpresetkeys}
\def\XKV@unpresetkeys{%
  \XKV@ifundefined{XKV@\XKV@header preseth}{%
    \XKV@err{no presets defined for `\XKV@header'}%
  }{%
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header preseth\endcsname\@undefined
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header presett\endcsname\@undefined
  }%
}
\def\savekeys{\XKV@stfalse\XKV@testoptb\XKV@savekeys}
\def\gsavekeys{\XKV@sttrue\XKV@testoptb\XKV@savekeys}
\def\XKV@savekeys#1{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@checksanitizeb{#1}\XKV@tempa
    \ifXKV@st\expandafter\global\fi\expandafter\def\csname XKV@%
      \XKV@header save\expandafter\endcsname\expandafter{\XKV@tempa}%
  }{%
    \expandafter\XKV@merge\csname XKV@\XKV@header
      save\endcsname{#1}\XKV@getsg
  }%
}
\def\delsavekeys{\XKV@stfalse\XKV@testoptb\XKV@delsavekeys}
\def\gdelsavekeys{\XKV@sttrue\XKV@testoptb\XKV@delsavekeys}
\def\XKV@delsavekeys#1{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@err{no save keys defined for `\XKV@header'}%
  }{%
    \expandafter\XKV@delete\csname XKV@\XKV@header
      save\endcsname{#1}\XKV@getsg
  }%
}
\def\unsavekeys{\XKV@stfalse\XKV@testoptb\XKV@unsavekeys}
\def\gunsavekeys{\XKV@sttrue\XKV@testoptb\XKV@unsavekeys}
\def\XKV@unsavekeys{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@err{no save keys defined for `\XKV@header'}%
  }{%
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header save\endcsname\@undefined
  }%
}
\def\setkeys{\XKV@testopta{\XKV@testoptc\XKV@setkeys}}
\long\def\XKV@setkeys[#1]#2{%
  \XKV@checksanitizea{#2}\XKV@resb
  \let\XKV@naa\@empty
  \XKV@for@o\XKV@resb\XKV@tempa{%
    \expandafter\XKV@g@tkeyname\XKV@tempa=\@nil\XKV@tempa
    \XKV@addtolist@x\XKV@naa\XKV@tempa
  }%
  \ifnum\XKV@depth=\z@\let\XKV@rm\@empty\fi
  \XKV@usepresetkeys{#1}{preseth}%
  \expandafter\XKV@s@tkeys\expandafter{\XKV@resb}{#1}%
  \XKV@usepresetkeys{#1}{presett}%
  \let\CurrentOption\@empty
}
\def\XKV@usepresetkeys#1#2{%
  \XKV@presettrue
  \XKV@for@eo\XKV@fams\XKV@tfam{%
    \XKV@makehd\XKV@tfam
    \XKV@ifundefined{XKV@\XKV@header#2}{}{%
      \XKV@toks\expandafter\expandafter\expandafter
        {\csname XKV@\XKV@header#2\endcsname}%
      \@expandtwoargs\XKV@s@tkeys{\the\XKV@toks}%
        {\XKV@naa\ifx\XKV@naa\@empty\else,\fi#1}%
    }%
  }%
  \XKV@presetfalse
}
\long\def\XKV@s@tkeys#1#2{%
  \XKV@sp@deflist\XKV@na{#2}%
  \XKV@for@n{#1}\CurrentOption{%
    \expandafter\XKV@s@tk@ys\CurrentOption==\@nil
  }%
}
\long\def\XKV@s@tk@ys#1=#2=#3\@nil{%
  \XKV@g@tkeyname#1=\@nil\XKV@tkey
  \expandafter\KV@@sp@def\expandafter\XKV@tkey\expandafter{\XKV@tkey}%
  \ifx\XKV@tkey\@empty
    \XKV@toks{#2}%
    \ifcat$\the\XKV@toks$\else
      \XKV@err{no key specified for value `\the\XKV@toks'}%
    \fi
  \else
    \@expandtwoargs\in@{,\XKV@tkey,}{,\XKV@na,}%
    \ifin@\else
      \XKV@knftrue
      \KV@@sp@def\XKV@tempa{#2}%
      \ifXKV@preset\XKV@s@tk@ys@{#3}\else
        \ifXKV@pl
          \XKV@for@eo\XKV@fams\XKV@tfam{%
            \XKV@makehd\XKV@tfam
            \XKV@s@tk@ys@{#3}%
          }%
        \else
          \XKV@whilist\XKV@fams\XKV@tfam\ifXKV@knf\fi{%
            \XKV@makehd\XKV@tfam
            \XKV@s@tk@ys@{#3}%
          }%
        \fi
      \fi
      \ifXKV@knf
        \ifXKV@inpox
          \ifx\XKV@doxs\relax
            \ifx\@currext\@clsextension\else
              \let\CurrentOption\XKV@tkey\@unknownoptionerror
            \fi
          \else\XKV@doxs\fi
        \else
          \ifXKV@st
            \XKV@addtolist@o\XKV@rm\CurrentOption
          \else
            \XKV@err{`\XKV@tkey' undefined in families `\XKV@fams'}%
          \fi
        \fi
      \else
        \ifXKV@inpox\ifx\XKV@testclass\XKV@documentclass
          \expandafter\XKV@useoption\expandafter{\CurrentOption}%
        \fi\fi
      \fi
    \fi
  \fi
}
\def\XKV@s@tk@ys@#1{%
  \XKV@ifundefined{\XKV@header\XKV@tkey}{}{%
    \XKV@knffalse
    \XKV@ifundefined{XKV@\XKV@header save}{}{%
      \expandafter\XKV@testsavekey\csname XKV@\XKV@header
        save\endcsname\XKV@tkey
    }%
    \ifXKV@rkv
      \ifXKV@sg\expandafter\global\fi\expandafter\let
        \csname XKV@\XKV@header\XKV@tkey @value\endcsname\XKV@tempa
    \fi
    \expandafter\XKV@replacepointers\expandafter{\XKV@tempa}%
    \ifx\@empty#1\@empty\XKV@afterelsefi
      \XKV@ifundefined{\XKV@header\XKV@tkey @default}{%
        \XKV@err{no value specified for key `\XKV@tkey'}%
      }{%
        \expandafter\expandafter\expandafter\XKV@default
          \csname\XKV@header\XKV@tkey @default\endcsname\@nil
      }%
    \else\XKV@afterfi
      \XKV@srstate{@\romannumeral\XKV@depth}{}%
      \csname\XKV@header\XKV@tkey\expandafter
        \endcsname\expandafter{\XKV@tempa}\relax
      \XKV@srstate{}{@\romannumeral\XKV@depth}%
    \fi
  }%
}
\def\XKV@testsavekey#1#2{%
  \ifXKV@rkv\else
    \XKV@for@o#1\XKV@resa{%
      \expandafter\XKV@ifcmd\expandafter{\XKV@resa}\global\XKV@resa{%
        \ifx#2\XKV@resa
          \XKV@rkvtrue\XKV@sgtrue
        \fi
      }{%
        \ifx#2\XKV@resa
          \XKV@rkvtrue\XKV@sgfalse
        \fi
      }%
    }%
  \fi
}
\long\def\XKV@replacepointers#1{%
  \let\XKV@tempa\@empty
  \let\XKV@resa\@empty
  \XKV@r@placepointers#1\usevalue\@nil
}
\long\def\XKV@r@placepointers#1\usevalue#2{%
  \XKV@addtomacro@n\XKV@tempa{#1}%
  \def\XKV@tempb{#2}%
  \ifx\XKV@tempb\@nnil\else\XKV@afterfi
    \XKV@ifundefined{XKV@\XKV@header#2@value}{%
      \XKV@err{no value recorded for key `#2'; ignored}%
      \XKV@r@placepointers
    }{%
      \@expandtwoargs\in@{,#2,}{,\XKV@resa,}%
      \ifin@\XKV@afterelsefi
        \XKV@err{back linking pointers; pointer replacement canceled}%
      \else\XKV@afterfi
        \XKV@addtolist@x\XKV@resa{#2}%
        \expandafter\expandafter\expandafter\XKV@r@placepointers
          \csname XKV@\XKV@header#2@value\endcsname
      \fi
    }%
  \fi
}
\def\XKV@default#1#2\@nil{%
  \expandafter\edef\expandafter\XKV@tempa
    \expandafter{\expandafter\@gobble\string#1}%
  \edef\XKV@tempb{\XKV@header\XKV@tkey}%
  \@onelevel@sanitize\XKV@tempb
  \ifx\XKV@tempa\XKV@tempb
    \begingroup
      \expandafter\def\csname\XKV@header\XKV@tkey\endcsname##1{%
        \gdef\XKV@tempa{##1}%
      }%
      \csname\XKV@header\XKV@tkey @default\endcsname
    \endgroup
    \XKV@ifundefined{XKV@\XKV@header save}{}{%
      \expandafter\XKV@testsavekey\csname XKV@\XKV@header
        save\endcsname\XKV@tkey
    }%
    \ifXKV@rkv
      \ifXKV@sg\expandafter\global\fi\expandafter\let
        \csname XKV@\XKV@header\XKV@tkey @value\endcsname\XKV@tempa
    \fi
    \expandafter\XKV@replacepointers\expandafter
      {\XKV@tempa}\XKV@afterelsefi
    \XKV@srstate{@\romannumeral\XKV@depth}{}%
    \expandafter#1\expandafter{\XKV@tempa}\relax
    \XKV@srstate{}{@\romannumeral\XKV@depth}%
  \else\XKV@afterfi
    \XKV@srstate{@\romannumeral\XKV@depth}{}%
    \csname\XKV@header\XKV@tkey @default\endcsname\relax
    \XKV@srstate{}{@\romannumeral\XKV@depth}%
  \fi
}
\def\setrmkeys{\XKV@testopta{\XKV@testoptc\XKV@setrmkeys}}
\def\XKV@setrmkeys[#1]{%
  \def\XKV@tempa{\XKV@setkeys[#1]}%
  \expandafter\XKV@tempa\expandafter{\XKV@rm}%
}
\XKVcatcodes
\endinput
%%
%% End of file `xkeyval.tex'.


==> xkvutils.tex <==
%%
%% This is file `xkvutils.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xkeyval.dtx  (with options: `xkvutils')
%% 
%% ---------------------------------------
%% Copyright (C) 2004-2014 Hendri Adriaens
%% ---------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2003/12/01 or later.
%%
%% This work has the LPPL maintenance status "maintained".
%%
%% This Current Maintainer of this work is Hendri Adriaens.
%%
%% This work consists of the file xkeyval.dtx and derived files
%% keyval.tex, xkvtxhdr.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvutils.tex, pst-xkey.tex, pst-xkey.sty, xkveca.cls,
%% xkvecb.cls, xkvesa.sty, xkvesb.sty, xkvesc.sty, xkvex1.tex,
%% xkvex2.tex, xkvex3.tex and xkvex4.tex.
%%
%% The following files constitute the xkeyval bundle and must be
%% distributed as a whole: readme, xkeyval.pdf, keyval.tex,
%% pst-xkey.sty, pst-xkey.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvtxhdr.tex, xkvutils.tex, pst-xkey.dtx and xkeyval.dtx.
%%
\csname XKeyValUtilsLoaded\endcsname
\let\XKeyValUtilsLoaded\endinput
\edef\XKeyValUtilsCatcodes{%
  \catcode`\noexpand\@\the\catcode`\@\relax
  \let\noexpand\XKeyValUtilsCatcodes\relax
}
\catcode`\@=11\relax
\newtoks\XKV@toks
\newtoks\XKV@tempa@toks
\long\def\@firstoftwo#1#2{#1}
\long\def\@secondoftwo#1#2{#2}
\long\def\XKV@afterfi#1\fi{\fi#1}
\long\def\XKV@afterelsefi#1\else#2\fi{\fi#1}
\ifx\ifcsname\@undefined\XKV@afterelsefi
  \def\XKV@ifundefined#1{%
    \begingroup\expandafter\expandafter\expandafter\endgroup
      \expandafter\ifx\csname#1\endcsname\relax
      \expandafter\@firstoftwo
    \else
      \expandafter\@secondoftwo
    \fi
  }
\else
  \def\XKV@ifundefined#1{%
    \ifcsname#1\endcsname
      \expandafter\@secondoftwo
    \else
      \expandafter\@firstoftwo
    \fi
  }
\fi
\XKV@ifundefined{ver@keyval.sty}{
  \input keyval
  \expandafter\def\csname ver@keyval.sty\endcsname{1999/03/16}
}{}
\long\def\@ifnextcharacter#1#2#3{%
  \@ifnextchar\bgroup
  {\@ifnextchar{#1}{#2}{#3}}%
  {\@ifncharacter{#1}{#2}{#3}}%
}
\long\def\@ifncharacter#1#2#3#4{%
  \if\string#1\string#4%
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
  {#2}{#3}#4%
}
\long\def\XKV@for@n#1#2#3{%
  \XKV@tempa@toks{#1}\edef#2{\the\XKV@tempa@toks}%
  \ifx#2\@empty
    \XKV@for@break
  \else
    \expandafter\XKV@f@r
  \fi
  #2{#3}#1,\@nil,%
}
\long\def\XKV@f@r#1#2#3,{%
  \XKV@tempa@toks{#3}\edef#1{\the\XKV@tempa@toks}%
  \ifx#1\@nnil
    \expandafter\@gobbletwo
  \else
    #2\expandafter\XKV@f@r
  \fi
  #1{#2}%
}
\long\def\XKV@for@break #1\@nil,{\fi}
\long\def\XKV@for@o#1{\expandafter\XKV@for@n\expandafter{#1}}
\long\def\XKV@for@en#1#2#3{\XKV@f@r#2{#3}#1,\@nil,}
\long\def\XKV@for@eo#1#2#3{%
  \def#2{\XKV@f@r#2{#3}}\expandafter#2#1,\@nil,%
}
\long\def\XKV@whilist#1#2#3\fi#4{%
  #3\expandafter\XKV@wh@list#1,\@nil,\@nil\@@#2#3\fi{#4}{}\fi
}
\long\def\XKV@wh@list#1,#2\@@#3#4\fi#5#6{%
  \def#3{#1}%
  \ifx#3\@nnil
    \def#3{#6}\expandafter\XKV@wh@l@st
  \else
    #4%
      #5\expandafter\expandafter\expandafter\XKV@wh@list
    \else
      \def#3{#6}\expandafter\expandafter\expandafter\XKV@wh@l@st
    \fi
  \fi
  #2\@@#3#4\fi{#5}{#1}%
}
\long\def\XKV@wh@l@st#1\@@#2#3\fi#4#5{}
\long\def\XKV@addtomacro@n#1#2{%
  \XKV@tempa@toks\expandafter{#1#2}%
  \edef#1{\the\XKV@tempa@toks}%
}
\def\XKV@addtomacro@o#1#2{%
  \expandafter\XKV@addtomacro@n\expandafter#1\expandafter{#2}%
}
\def\XKV@addtolist@n#1#2{%
  \ifx#1\@empty
    \XKV@addtomacro@n#1{#2}%
  \else
    \XKV@addtomacro@n#1{,#2}%
  \fi
}
\def\XKV@addtolist@o#1#2{%
  \ifx#1\@empty
    \XKV@addtomacro@o#1#2%
  \else
    \XKV@addtomacro@o#1{\expandafter,#2}%
  \fi
}
\def\XKV@addtolist@x#1#2{\edef#1{#1\ifx#1\@empty\else,\fi#2}}
\def\@selective@sanitize{\@testopt\@s@lective@sanitize\@M}
\def\@s@lective@sanitize[#1]#2#3{%
  \begingroup
    \count@#1\relax\advance\count@\@ne
    \XKV@toks\expandafter{#3}%
    \def#3{#2}\@onelevel@sanitize#3%
    \edef#3{{#3}{\the\XKV@toks}}%
    \expandafter\@s@l@ctive@sanitize\expandafter#3#3%
    \expandafter\XKV@tempa@toks\expandafter{#3}%
  \expandafter\endgroup\expandafter\toks@\expandafter{\the\XKV@tempa@toks}%
  \edef#3{\the\toks@}%
}
\def\@s@l@ctive@sanitize#1#2#3{%
  \def\@i{\futurelet\@@tok\@ii}%
  \def\@ii{%
    \expandafter\@iii\meaning\@@tok\relax
    \ifx\@@tok\@s@l@ctive@sanitize
      \let\@@cmd\@gobble
    \else
      \ifx\@@tok\@sptoken
        \XKV@toks\expandafter{#1}\edef#1{\the\XKV@toks\space}%
        \def\@@cmd{\afterassignment\@i\let\@@tok= }%
      \else
        \let\@@cmd\@iv
      \fi
    \fi
    \@@cmd
  }%
  \def\@iii##1##2\relax{\if##1\@backslashchar\let\@@tok\relax\fi}%
  \def\@iv##1{%
    \toks@\expandafter{#1}\XKV@toks{##1}%
    \ifx\@@tok\bgroup
      \advance\count@\m@ne
      \ifnum\count@>\z@
        \begingroup
          \def#1{\expandafter\@s@l@ctive@sanitize
            \csname\string#1\endcsname{#2}}%
          \expandafter#1\expandafter{\the\XKV@toks}%
          \XKV@toks\expandafter\expandafter\expandafter
            {\csname\string#1\endcsname}%
          \edef#1{\noexpand\XKV@toks{\the\XKV@toks}}%
        \expandafter\endgroup#1%
      \fi
      \edef#1{\the\toks@{\the\XKV@toks}}%
      \advance\count@\@ne
      \let\@@cmd\@i
    \else
      \edef#1{\expandafter\string\the\XKV@toks}%
      \expandafter\in@\expandafter{#1}{#2}%
      \edef#1{\the\toks@\ifin@#1\else
              \ifx\@@tok\@sptoken\space\else\the\XKV@toks\fi\fi}%
      \edef\@@cmd{\noexpand\@i\ifx\@@tok\@sptoken\the\XKV@toks\fi}%
    \fi
    \@@cmd
  }%
  \let#1\@empty\@i#3\@s@l@ctive@sanitize
}
\long\def\XKV@checksanitizea#1#2{%
  \XKV@ch@cksanitize{#1}#2=%
  \ifin@\else\XKV@ch@cksanitize{#1}#2,\fi
  \ifin@\@selective@sanitize[0]{,=}#2\fi
}
\def\XKV@checksanitizeb#1#2{%
  \XKV@ch@cksanitize{#1}#2,%
  \ifin@\@selective@sanitize[0],#2\fi
}
\long\def\XKV@ch@cksanitize#1#2#3{%
  \XKV@tempa@toks{#1}\edef#2{\the\XKV@tempa@toks}%
  \@onelevel@sanitize#2%
  \@expandtwoargs\in@#3{#2}%
  \ifin@
    \long\def#2##1#3##2\@nil{%
      \XKV@tempa@toks{##2}\edef#2{\the\XKV@tempa@toks}%
      \ifx#2\@empty\else\in@false\fi
    }%
    #2#1#3\@nil
  \fi
  \XKV@tempa@toks{#1}\edef#2{\the\XKV@tempa@toks}%
}
\def\XKV@sp@deflist#1#2{%
  \let#1\@empty
  \XKV@for@n{#2}\XKV@resa{%
    \expandafter\KV@@sp@def\expandafter\XKV@resa\expandafter{\XKV@resa}%
    \XKV@addtomacro@o#1{\expandafter,\XKV@resa}%
  }%
  \ifx#1\@empty\else
    \def\XKV@resa,##1\@nil{\def#1{##1}}%
    \expandafter\XKV@resa#1\@nil
  \fi
}
\def\XKV@merge#1#2#3{%
  \XKV@checksanitizea{#2}\XKV@tempa
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \XKV@pltrue
    #3\XKV@tempa\XKV@tempb
    \let\XKV@tempc#1%
    \let#1\@empty
    \XKV@for@o\XKV@tempc\XKV@tempc{%
      #3\XKV@tempc\XKV@tempd
      \ifx\XKV@tempb\XKV@tempd
        \XKV@plfalse
        \XKV@addtolist@o#1\XKV@tempa
      \else
        \XKV@addtolist@o#1\XKV@tempc
      \fi
    }%
    \ifXKV@pl\XKV@addtolist@o#1\XKV@tempa\fi
  }%
  \ifXKV@st\global\let#1#1\fi
}
\def\XKV@delete#1#2#3{%
  \XKV@checksanitizeb{#2}\XKV@tempa
  \let\XKV@tempb#1%
  \let#1\@empty
  \XKV@for@o\XKV@tempb\XKV@tempb{%
    #3\XKV@tempb\XKV@tempc
    \@expandtwoargs\in@{,\XKV@tempc,}{,\XKV@tempa,}%
    \ifin@\else\XKV@addtolist@o#1\XKV@tempb\fi
  }%
  \ifXKV@st\global\let#1#1\fi
}
\XKeyValUtilsCatcodes
\endinput
%%
%% End of file `xkvutils.tex'.

